On the Explanatory Power of Decision Trees

Decision trees have long been recognized as models of choice in sensitive applications where interpretability is of paramount importance. In this paper, we examine the computational ability of Boolean decision trees in deriving, minimizing, and counting sufficient reasons and contrastive explanations. We prove that the set of all sufficient reasons of minimal size for an instance given a decision tree can be exponentially larger than the size of the input (the instance and the decision tree). Therefore, generating the full set of sufficient reasons can be out of reach. In addition, computing a single sufficient reason does not prove enough in general; indeed, two sufficient reasons for the same instance may differ on many features. To deal with this issue and generate synthetic views of the set of all sufficient reasons, we introduce the notions of relevant features and of necessary features that characterize the (possibly negated) features appearing in at least one or in every sufficient reason, and we show that they can be computed in polynomial time. We also introduce the notion of explanatory importance, that indicates how frequent each (possibly negated) feature is in the set of all sufficient reasons. We show how the explanatory importance of a feature and the number of sufficient reasons can be obtained via a model counting operation, which turns out to be practical in many cases. We also explain how to enumerate sufficient reasons of minimal size. We finally show that, unlike sufficient reasons, the set of all contrastive explanations for an instance given a decision tree can be derived, minimized and counted in polynomial time.

==> abstract.tex <==
%Decision trees are popular ML models for the classification task because they are usually considered as highly interpretable.
%Indeed, for any instance to be classified using a decision tree, one can easily determine a subset of its characteristics that
%prove sufficient to explain the classification that is achieved. An irredundant subset of characteristics, called a sufficient reason, 
%can also be computed efficiently from the given instance. However, a sufficient reason is not guaranteed to be intelligible
%because it may contain too many characteristics and/or characteristics that are not comprehensible by the explainee.
%To deal with this issue, we present several refinements / generalizations of the notion of sufficient reasons.
%We identify the complexity of computing such reasons for a given instance when the classifier is a decision tree, 
%and we describe exact or approximate algorithms for deriving them.  We also present
%empirical results for illustrating the gain in intelligibility they may offer and 
%the performances of the algorithms for computing them. 

Decision trees are popular ML models for the classification task because they are usually considered as highly interpretable.
Indeed, for any instance to be classified using a decision tree, one can easily determine a subset of its features in order 
to explain the classification that is achieved. An irredundant subset of features, called a sufficient reason, 
can also be computed efficiently from the given instance. However, sufficient reasons are not guaranteed to be intelligible
because they may contain too many features. 
In order to deal with this issue, we present a refinement and a generalization of the notion of sufficient reasons. 
We identify the complexity of computing such reasons for a given instance when the classifier is a decision tree, 
and we describe and evaluate algorithms for deriving them.  
%We also present empirical results for illustrating the gain in intelligibility they may offer and the performances of the algorithms for computing them. 


==> beyond.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Beyond Sufficient Reasons}\label{beyond}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Minimal Reasons}

Since conciseness is often a desirable property of explanations, a natural way for improving the clarity of 
sufficient reasons is to focus on the shortest ones:

\begin{definition}[Minimal Reason] 
    Let $f \in \mathcal F_n$ and $\vec x \in \{0,1\}^n$ such that $f(\vec x) = 1$.
    A \emph{minimal reason} for $\vec x$ given $f$ is a sufficient reason for $\vec x$ given $f$ that contains a minimal number
    of literals.
\end{definition}

\begin{example} Based on our running example, $x_1 \wedge x_4$ is a minimal reason for $\vec x$ given $T$, 
    while $x_2 \wedge x_3 \wedge x_4$ is not.
\end{example}

Importantly, \emph{minimal reasons} should not to be confused with \emph{minimum-cardinality explanations}  \cite{ShihCD18},
where the minimality condition bears on the features set to $1$ in the input instance. 
In fact, as a direct by-product of Proposition 8 from \cite{Audemardetal20}, 
computing a minimum-cardinality explanation for an input instance $\vec x$ given a decision tree $T$
can be done in polynomial-time. Unfortunately, this is not the case for minimal reasons, 
which are computationally more demanding:

\begin{proposition}\label{prop:minimalreasonDT}
    Let $T \in \dt_n$ and $\vec x \in \{0,1\}^n$ such that $T(\vec x) = 1$.
    Computing a minimal reason for $\vec x$ given $T$
    is {\sf NP}-hard.
  \end{proposition}
  
A source of complexity that may explain this hardness result is the number of sufficient reasons for an input instance $\vec x$,
which can be exponential in the size of the decision tree at hand.
Indeed, even for the restricted class of decision trees with
logarithmic depth, an input instance can have exponentially many sufficient reasons:

\begin{proposition}\label{prop:nbDT}
There is a decision tree $T \in\dt_n$ of depth $\log_2(n + 1)$ 
 such that for any $\vec x \in \{0,1\}^n$, the number of sufficient reasons for $\vec x$ given $T$ is at least 
 $\lfloor \frac{3}{2}^{\frac{n + 1}{2}} \rfloor$. 
\end{proposition}

A common approach for handling {\sf NP}-optimization problems is to rely on modern constraint solvers.
One follows this direction here and casts the task of finding minimal reasons as a Boolean constraint optimization problem. 
We first need to recall that a \textsc{Partial MaxSAT} problem consists of a pair  $(C_{\mathrm{soft}}, C_{\mathrm{hard}})$
of \cnf\ formulae, and the goal is to find a Boolean assignment that satisfies a maximum number of 
clauses in $C_{\mathrm{soft}}$, while satisfying all clauses in $C_{\mathrm{hard}}$.

\begin{proposition}\label{prop:minimaloptim}
    Let $T$ be a decision tree in $\dt_n$ and $\vec x \in \{0,1\}^n$ be an instance such that $T(\vec x) = 1$. 
    Let $(C_{\mathrm{soft}}, C_{\mathrm{hard}})$ be an instance of the \textsc{Partial MaxSAT} problem such that:
    \begin{align*}
        C_{\mathrm{soft}} &= \{\overline x_i  : x_i \in t_{\vec x}\} \cup \{x_i  : \overline x_i \in t_{\vec x}\} \\
        C_{\mathrm{hard}} &= \{c_{\mid \vec x} : c \in \cnf(T) \} 
    \end{align*}
    where $c_{\mid \vec x} = c \cap t_{\vec x}$ is the restriction of $c$ to the literals in $t_{\vec x}$.
    Any optimal solution of $(C_{\mathrm{hard}}, C_{\mathrm{soft}})$ is a minimal reason for $\vec x$ given $T$.
\end{proposition}

As an alternative to \textsc{Partial MaxSAT} solving, we may explore the possibility of finding good approximations 
of minimal reasons in polynomial-time. 
For decision trees, this task can be cast as a \textsc{Min Hitting Set} problem: given a representation $T \in \dt_n$ 
and an instance $\vec x \in \{0,1\}^n$ such that $T(\vec x) = 1$, let $H_{\vec x}(T)$ be the hypergraph formed by
the set of vertices $t_{\vec x}$ and the set of hyperedges $\{c_{\mid \vec x} : c \in \cnf(T)\}$.
By construction, $t$ is a minimal reason for $\vec x$ given $T$ if and only if $t$ is a minimal hitting set of $H_{\vec x}(T)$.
Based on this equivalence, the task of finding minimal reasons can be approximated using the following 
\emph{greedy covering algorithm}: starting from $t = \emptyset$, iteratively add to $t$ a vertex $l_i \in t_{\vec x}$ 
of maximal degree, and removes it together with all 
adjacent hyperedges in $H_{\vec x}(T)$. Based on the performance analysis of the greedy covering algorithm \cite{SLAVIK1997},
the size of the final term $t$ is at most $\ln n - \ln\ln n + 0.78$ larger than the size of a minimal reason for $\vec x$ given $T$.
To sum up:


\begin{proposition}\label{prop:approximable}
    Let $T \in \dt_n$, and $\vec x \in \{0,1\}^n$ such that $T(\vec x) = 1$. 
    Computing a minimal reason for $\vec x$ given $T$ is approximable to within a ratio of $\ln n - \ln\ln n + \Theta(1)$. 
\end{proposition}

% Indeed, the greedy covering algorithm is guaranteed to output a term $t$ such that $|t|$ is at most $\ln n - \ln\ln n + c$ larger
% than the size of a minimal reason for $\vec x$ given $T$ (where $c$ is a fixed constant).

% the following result directly follows from the performance analysis of the well-known greedy algorithm for 
% \textsc{Min Hitting Set}\footnote{This is trivially equivalent to the \textsc{Min Set Cover} problem by changing the role of vertices and edges.} 
% \cite{SLAVIK1997}.
% adjacent hyperedges in $H_{\vec x}(T)$. Let $\mathrm{adj}(l_i)$ be the set of vertices in $H_{\vec x}(T)$ which are adjacent to $l_i$, 
% and let $A = \max_{i=1}^n \size{\mathrm{adj}(l_i)}$. Note that for the \cnf\ encoding of decision trees, 
% $A$ often coincides with the depth of the tree. Based on the analysis of greedy covering algorithm \cite{SLAVIK1997,OKUN2005}, we get the following result. 


%\pierre{Si on sait étendre l'algo exact et l'algo approché au cas où la préférence est donnée par une fonction de coût (minimal-weight reason), c'est ici qu'il faut mettre les résultats.}
%Nevertheless, both exact and approximation algorithms can be defined for the purpose of deriving a minimal reason, and more generally, a ``preferred'' reason
%where preference is captured as minimality w.r.t. a fully additive, linear utility function. In this case, features can have distinct weights (minimal reasons correspond to the specific case when all weights are equal).
%
%Our exact algorithm is based on MAX-SAT encoding and the use of a MAX-SAT solver. Obviously enough, this algorithm does not run in polynomial time in the worst case, but due to the tremendous progress in SAT solving achieved during the past two decades, experiments show that it can solve instances of ``reasonable'' sizes in practice (see Section \ref{experiments}). The approximation algorithm runs in polynomial time in the size of the input and guarantees that the computed reason
%as a size that is close to the one of a minimal reason. 
%\pierre{Present the reduction to MAX-SAT. Introduce a proposition establishing the correctness of the encoding.}
%\pierre{Present the approximation algorithm for minimal reasons. Introduce a proposition establishing the approximation bound.}

%As a consequence of Proposition \ref{prop:minimalreasonDT}, the algorithm for pointing out in polynomial time a sufficient reason 
%cannot be extended to the issue of selecting
%a ``preferred'' reason from the sufficient ones when any preference relation is considered. 
%%Especially, as we will see next, computing a reason that contains as few features
%%as possible cannot be achieved in polynomial time unless {\sf P = NP}. The search for a ``preferred reason''
%%among the sufficient reasons cannot always be done efficiently. 
%Note that a straightforward generate-and-test algorithm would not be not
%convenient to reach the goal because the search space (i.e., the set of all sufficient reasons) is of exponential size
%in the worst case.
%%For the classes of \cnf\ and \dnf\ formulas, it is well-known that an input instance can have exponentially many sufficient reasons.
%%For example, the monotone \cnf\ formula $F = \bigwedge_{i=1}^{\lfloor\frac{n}{2}\rfloor} (x_{2i-1} \vee x_{2i})$ has $2^{\lfloor\frac{n}{2}\rfloor}$.
%%prime implicants, each of them being implied by $\vec x = (1,1,\cdots,1)$. Surprisingly, 
%Indeed, even for the restricted class of decision trees of 
%logarithmic depth, an input instance can have exponentially many sufficient reasons:
%
%\begin{proposition}\label{prop:nbDT}
%    Let $\dt^k_{n}$ be the class of decision trees of depth $k \geq 1$ over $n = 2^k - 1$ variables. Then, there is a decision tree $T \in \dt^k_{n}$ 
%    such that for any input instance $\vec x \in \{0,1\}^n$, the number of sufficient reasons for $\vec x$ given $T$ is at least $\lfloor \frac{3}{2}^{\frac{n + 1}{2}} \rfloor$. 
%\end{proposition}

% Fred: tout ceci est completement trivial et n'a aucun interet pour NIPS.
%\subsection{Comprehensible Reasons}

% Sufficient reasons 
% are not always guaranteed to be ``intelligible''. 
% Indeed, it can be the case that some features in the prime implicant 
% are not understandable by the user to which the explanation is supplied. 
% This calls for a notion of \emph{comprehensible reason}:
%
%% Fred: l'exemple médical est intéressant, mais pas sûr qu'on ait la place.
%% In some cases, limiting the size of an explanation to a few literals is not enough 
%% to ensure that the explanation is intelligible \cite{CosteMarquis20}.
%% Indeed, it can be the case that some of the features in the explanation are not understandable by the user to which the explanation
%% must be reported. 
%%This happens, for example, when trying to predict diseases from observed symptoms and physiological measures
%%associated with patients: though the fact that the erythrocyte sedimentation rate in a blood test is over a given threshold is a
%%meaningful piece of information for a physician, for many people this will be meaningless.
%
%\begin{definition}[Comprehensible Reason] 
%    Let $f \in \mathcal F_n$ and $\vec x \in \{0,1\}^n$ such that $f(\vec x) = 1$.
%    In addition, let $I \subseteq X_n$ be a subset of intelligible features. 
%    Then, a \emph{comprehensible reason} for $\vec x$ given $f$ is a sufficient reason for $\vec x$ given $f$ that contains only literals built up from $I$.
%\end{definition}
%
%\begin{example} Suppose that the user does not understand what \emph{sympodial}\footnote{An orchid is sympodial when it grows sideways.} (feature $x_4$) means.
% Is it possible to find a sufficient reason for $\vec x$ given $T$ that does not include $x_4$? 
%    Obviously, the answer is negative because $x_4$ is \emph{mandatory} for the {\it Cattleya} classifier $T$, that is, any sufficient reason 
%    for any input instance must include a literal on $x_4$. 
%\end{example}
%
%As illustrated in the above example, a key issue for deriving ``intelligible'' reasons is to determine whether at least one comprehensible reason exists, 
%depending on the choice of $I$. Interestingly, this problem is tractable for decision trees: 
%
%\begin{proposition} \label{prop:understandablereasonDT}
%    Let $T \in \dt_n$ and $\vec x \in \{0,1\}^n$ such that $f(\vec x) = 1$. 
%    Then, for any set $I \subseteq X_n$ of intelligible features, deciding whether a comprehensible reason for $\vec x$ given $T$
%    exists, and deriving such a reason when this is the case, can be done in $\mathcal O(n \size{T})$ time.
%\end{proposition}
%
%\fred{Est-ce qu'on pourrait generaliser aux delta-probable comprehensible reasons? ... Cela reste poly, mais c'est une consequence de 3 \& 4.}
%\pierre{Oui, j'ai ajouté une phrase dans la partie "Probabilistic Reasons"}
%
%%\color{blue}
%%\pierre{J'ai remis la suite (partie en bleu). Merci de le mettre éventuellement en commentaires mais de ne pas l'effacer sinon cela m'oblige à retaper
%%des trucs et je risque d'introduire des erreurs.}
%%\fred{OK Pierre}
%

\fred{A reprendre complètement.}
\subsection{Preferred Reasons}

The user may also have some expectations about the features that should be present in explanations. 
For instance, she might consider that some features are more important than others for explaining decisions. 
The reason that is derived should cohere as much as possible to the user's expectations or \emph{confirmation bias}.\footnote{Confirmation bias is the tendency to search for, 
interpret, favor, and recall information in a way that confirms or supports one's prior beliefs or values. Since the 1960's, many experiments in psychology and cognitive science 
people have shown that people are biased toward confirming their existing beliefs (see e.g., \cite{Oswaldetal04}).}
However, when computing a sufficient reason, even a comprehensible one, we cannot guarantee that a ``better'' reason 
for the user would not exist. 

To make it more formal, one needs a notion of \emph{``preferred''} sufficient reason. Depending on the preference model at hand, the
computation of a single preferred reason can be intractable (as we will see soon). Fortunately, there are preference models for which
intractability can be avoided. 
Especially, this is the case when the preference relation is ordinal and based on a total preorder $\leq$ over $X_n$,
such that $x_i \leq x_j$ means that feature $x_i$ is considered as less important or less expected than feature $x_j$. 
$\leq$ can be represented by a \emph{prioritization} (or stratification) of $X_n$, i.e., 
an ordered partition $C_1, \ldots, C_p$ of the features from $X_n$ such that $x_i$ and $x_j$ belongs to the
same set of the partition if and only if $x_i \leq x_j$ and $x_j \leq x_i$, and $C_i$ precedes $C_j$ in the partition (i.e., $i < j$) whenever
every element of $C_i$ is before every element of $C_j$ w.r.t. $\leq$. Whatever $C$ among $C_1, \ldots, C_p$ and a term $t$ over $X_n$,
$t[C]$ denotes the term composed of the literals of $t$ that are over variables from $C$.

Based on the prioritization $C_1, \ldots, C_p$ of $X_n$ induced by $\leq$, one can define a preference relation $\sqsubset$ on the terms 
over $X_n$ by stating that $t \sqsubset t'$ if and only if $\exists i \in \{1, \ldots, p\} \forall j \in \{1, \ldots, i-1\}$, $t[C_j] = t'[C_j]$ and 
$t[C_i] \subset t'[C_i]$.\footnote{The construction is reminiscent to the one used for characterizing preferred subtheories in \cite{Brewka89}.}
It can be checked that $\sqsubset$ is a strict, partial order (i.e., an irreflexive and transitive relation). 
Given a set of terms, the minimal ones w.r.t. $\sqsubset$ correspond intuitively to those that contain as few unexpected literals
as possible (where the comparison is based on set inclusion). On this ground, we are now ready to define the notion of inclusion-preferred reason:

\begin{definition}[Inclusion-Preferred Reason] 
   Let $f \in \mathcal F_n$, $\leq$ a total preorder over $X_n$, and $\vec x \in \{0,1\}^n$ be an instance such that $f(\vec x) = 1$.
   Then, an \emph{inclusion-preferred reason} for $\vec x$ given $f$ is a sufficient reason $t$ for $\vec x$ given $f$ 
   such that there is no sufficient reason $t'$ for $\vec x$ given $f$ satisfying $t' \sqsubset t$.
\end{definition}

\begin{example}[Example \ref{running-ex} cont'ed]
Suppose that the expectations of the explainee correspond to the prioritization $\{x_4\}, \{x_3, x_2\}, \{x_5\}, \{x_1\}$ reflecting the fact
that having fragrant flowers is, for her/him, a more salient aspect of {\it Cattleya} orchids than the other features.
% (especially than $d$ that she/he does not understand). 
Then $x_1 \wedge x_4$ is an inclusion-preferred reason for $\vec x$ given $T$, while $x_2 \wedge x_3 \wedge x_4$ is not because 
$x_1 \wedge x_4 \sqsubset x_2 \wedge x_3 \wedge x_4$ holds.
\end{example}

The greedy algorithm presented above for generating one sufficient reason can be cast in such a way that it generates
an inclusion-preferred reason for an instance given a decision tree:

\begin{proposition} \label{prop:favoritereasonDT}
   Let $T \in \dt_n$, $\leq$ be a total preorder over $X_n$, and $\vec x \in \{0,1\}^n$. 
   Then, deriving an inclusion-preferred reason for $\vec x$ given $T$ and $\leq$ can be done in $\mathcal O(\size{G} + n \size{T})$ time
   where $G$ is the graph $(X_n, \leq)$.
\end{proposition}
\color{black}

\pierre{J'ai remis la suite comme elle était.}
To make it more formal, one needs a notion of \emph{preferred} sufficient reason. Depending on the preference model at hand, the
computation of a single preferred reason can be intractable. Fortunately, there are preference models for which
intractability can be avoided. This is especially the case when preferences over features can be captured by a utility function 
$u: X_n \rightarrow \R$, where $u(x_i) < u(x_j)$ indicates that $x_i$ is less preferred than $x_j$.\pierre{Euh, non, ce n'est pas traitable
dans ce cas-là, on l'a montré avec les minimal reasons qui est un cas particulier de ``preferred reason'' où tous les $x_i$ ont des
poids égaux non nuls. A revoir.}
Based on this additive model, the utility of a term $t$ is given by $u(t) = \sum_{x_i \in \Var{t}} u(x_i)$.  

\begin{definition}[Minimal-Weight Reason] 
   Let $f \in \mathcal F_n$, $u: X_n \rightarrow \R$ be a utility function, and $\vec x \in \{0,1\}^n$ 
   be an instance such that $f(\vec x) = 1$. Then, a \emph{minimal-weight reason} for $\vec x$ given $f$ is a sufficient reason 
   $t$ for $\vec x$ given $f$ such that $u(t)$ is maximal.
\end{definition}
\pierre{J'appellerais plutôt cela des minimal-weight reasons pour garder ``preferred reason'' comme le terme générique. Je pense qu'il faut regrouper tout ce qui suit avec les minimal reasons
car les minimal-weight reasons les généralisent et les algos exacts et approchés à base de partial-weighted-MAX-SAT s'appliquent de facon générale aux minimal-weight reasons si j'ai bien tout compris}


\begin{proposition}\label{prop:minimalreasonDT}
   Let $T \in \dt_{n}$ and $\vec x \in \{0,1\}^n$ such that $T(\vec x) = 1$.
   Unless {\sf P = NP}, there is no polynomial-time algorithm for computing a minimal reason for $\vec x$ given $T$.
\end{proposition}

Nevertheless, both exact and approximation algorithms can be defined for the purpose of deriving a minimal reason
by casting this task as a \textsc{Minimal Hitting Set} problem:

\begin{proposition}\label{prop:MHS}
   Let $T \in \dt_{n}$, and $\vec x \in \{0,1\}^n$ such that $T(\vec x) = 1$.
   Let $H_{\vec x}(T)$ be the hypergraph formed by
   the set of vertices $t_{\vec x}$ and the set of hyperedges $\{c \cap t_{\vec x}: c \in \cnf(T)\}$.
   Then, $t$ is a minimal reason for $\vec x$ given $T$ if and only if $t$ is a minimal hitting set of $H_{\vec x}(T)$.
\end{proposition}

Based on this proposition, the task of finding minimal reasons can be encoded into a \textsc{Partial MAX-SAT} problem,
where the collection of hard clauses (which must be satisfied) is the set of hyperedges in $H_{\vec x}(T)$, and the 
set of soft clauses (which can be violated) is $\{\neg l_i : l_i \in t_{\vec x}\}$.
Obviously enough, a \textsc{Partial MAX-SAT} algorithm for this task does not run in polynomial time in the worst case, but due to the tremendous progress in \textsc{SAT} solving achieved during the past two decades since the advent of the CDCL architecture, 
experiments show that, in practice, the algorithm finds minimal reasons in a reasonable amount of time (see Section \ref{experiments}). 
%\footnote{The existence of such an algorithm would prove {\sf P = NP}.} -> Pour IJCAI, on n'a pas vraiment besoin de le préciser :-)


==> conclusion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusion}\label{conclusion}

%\pierre{TBC. Recall the main contributions and give some perspectives. Studying the case of random forests. Computing all the reasons.} 
%
%It is acknowledged that intelligibility is among the research questions pertaining to XAI that have not been 
%explored in depth, and that it should receive more attention  \cite{doshivelez2017rigorous,GuidottiMRTGP19}. Our work contributes 
%to fill the gap, with the study of the intelligibility of explanations when the predictions come from a decision tree
%and the design and analysis of some notions of reasons that refine or extend the notion of sufficient reason in this case.


It is acknowledged that intelligibility is among the research questions pertaining to XAI that have not been 
explored in depth, and that it should receive more attention  \cite{doshivelez2017rigorous,GuidottiMRTGP19}. Our work contributes 
to fill the gap, with a study of the intelligibility question for decision trees based on the sizes of the reasons.

Though it is possible to derive in polynomial time a sufficient reason for a given instance $\vec x$ when the classifier is a decision tree,
we have argued that such a reason cannot be guaranteed as intelligible in the general case because it may contain too many 
features. In order to deal with this issue, we have focused on a refinement and on a generalization of the notion of sufficient reasons, 
namely the minimal reasons and the probable reasons, respectively.
We have identified the complexity of computing such reasons for a given instance when the classifier is a decision tree, 
and we have described exact or approximate algorithms for deriving them.  
%Though the derivation of a sufficient reason for any given instance
%is tractable for both ML models, decision trees can be considered as more interpretable than random forests in the sense that deriving
% (or approximating) minimal or probable reasons looks more amenable for the former than for the latter.
We have also presented empirical results for illustrating the gain in intelligibility minimal reasons and probable reasons may offer, as well as  
the performances of the algorithms that have been pointed out for computing them.

Interestingly, unlike direct reasons that are specific to decision trees, the notions of minimal reasons and of $\delta$-probable reasons make sense for any
Boolean classifier (just as sufficient reasons do). Since, by construction, minimal reasons and $\delta$-probable reasons cannot be larger than
sufficient reasons, they appear as valuable concepts to the purpose of getting more intelligible explanations for the classifications made.
In the case of decision trees, all those reasons are in practice much smaller than the instances themselves. Though the most significant reduction
w.r.t. the size of the instances is achieved by the direct reasons, our experiments revealed that some further reduction can take place when
considering minimal reasons or $\delta$-probable reasons instead. In addition, in light of our experiments, 
the derivation of minimal reasons or of $\delta$-probable reasons does not require a tremendous computational effort.
The reduction they can lead to is thus almost for free.

%By construction, the resulting explanations cannot be larger than the direct reasons, and as such, 
%they are at least as intelligible as the reasons computed directly from decision trees. 

This work paves the way for some further developments. Identifying the complexity of deriving minimal reasons or $\delta$-probable reasons
for other Boolean classifiers, and developing and evaluating algorithms to compute such reasons is is a perspective we will 
consider in the near future. Exploiting pieces of knowledge to simplify the reasons during their computation is another research 
direction we plan to follow.

%Yet, our experimental results have revealed that whenever a direct reason is too large, 
%we can always find a minimal reason or several probable reasons (by varying $\delta$) in almost real-time.  
%Furthermore, when the binary features generated by the splitting rule in the decision tree learner are inter-connected via some domain theory,
%sufficient, minimal and probable reasons could be further simplified by leveraging this theory. 
%Designing and evaluating algorithms that compute reasons
%while taking advantage of such background knowledge is a perspective for further research we plan to investigate in the near future.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%\section*{Acknowledgements}
%
%%Many thanks to the anonymous reviewers for their comments and suggestions. 
%This work has benefited from the support of the AI Chair EXPE\textcolor{orange}{KC}TATION (ANR-19-CHIA-0005-01) of the French National Research Agency (ANR).
%It was also partially supported by TAILOR, a project funded by EU Horizon 2020 research
%and innovation programme under GA No 952215.


==> experiments.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experiments}\label{experiments}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%After an excursion into the theoretical aspects of this study, we are now in position to present the experimental results.
We have performed a number of experiments in order (i) to evaluate the practical performance of the algorithms for computing 
sufficient, minimal and $\delta$-probable reasons, and (ii) to assess the gain in intelligibility 
that results from focusing on the size of these different reasons, relatively to the size of direct reasons. 
%, in comparison with the size of direct reasons. 
%Since we wanted to consider only standard benchmarks, we did not make experiments regarding comprehensible reasons or inclusion-preferred reasons (additional metadata would have been required to do so).

\subsection{Empirical setting}
%\color{magenta}

\begin{table*}
\begin{scriptsize}
\begin{center}
 \begin{tabular}{lrrrrrrrrrrrr}
 \toprule
 % I Instances - F features - A Accuracy - N nb nodes - MD MaxDeph - #B nb bin
Dataset	&\#I	&\#F	&\%A	&\#N	&\#MD	&\#B	& \#DR	& \#SR	& \#MR	& \#95-PR	& \#90-PR	& \#75-PR\\
\midrule
 Ad-data	&3279	&1558	&96.58	&321.4	&85.2	&141.1	&33.8$\pm$14.9	&30.3$\pm$10.7	&28.8$\pm$9.9	&29.5$\pm$10.5	&28.3$\pm$10.2	&22.0$\pm$7.8\\
Adult	&48842	&14	&81.41	&12926.0	&47.4	&2973.2	&17.4$\pm$5.9	&16.5$\pm$5.1	&16.5$\pm$5.1	&16.3$\pm$5.2	&15.7$\pm$5.1	&12.9$\pm$4.5\\
AllBooks	&590	&8266	&71.02	&183.4	&42.9	&88.8	&15.0$\pm$13.5	&14.1$\pm$12.1	&14.1$\pm$12.1	&13.9$\pm$11.8	&13.8$\pm$11.7	&13.1$\pm$11.3\\
Arcene	&200	&10000	&73.00	&24.4	&5.3	&11.7	&4.1$\pm$0.9	&4.1$\pm$0.9	&4.1$\pm$0.9	&4.0$\pm$0.9	&3.9$\pm$0.9	&2.9$\pm$1.0\\
Christine	&5418	&1636	&62.77	&839.0	&34.3	&419.0	&16.1$\pm$9.1	&15.8$\pm$9.1	&15.8$\pm$9.1	&15.8$\pm$9.1	&15.7$\pm$9.1	&14.2$\pm$9.2\\
CNAE	&1079	&856	&86.00	&278.6	&52.5	&113.9	&14.5$\pm$13.7	&13.7$\pm$12.5	&13.7$\pm$12.5	&13.7$\pm$12.5	&13.7$\pm$12.4	&13.2$\pm$12.2\\
Dexter	&600	&20000	&86.50	&73.4	&12.7	&36.2	&7.2$\pm$2.8	&6.9$\pm$2.8	&6.9$\pm$2.8	&6.7$\pm$2.7	&6.5$\pm$2.7	&5.4$\pm$2.7\\
Dorothea	&1150	&100000	&90.70	&65.2	&18.8	&32.1&16.7$\pm$3.9	&16.6$\pm$4.2	&16.6$\pm$4.2	&16.4$\pm$4.2	&16.4$\pm$4.3	&14.8$\pm$4.1\\
Farm-ads	&4143	&54877	&86.75	&543.2	&91.3	&264.6	&25.9$\pm$21.4	&24.7$\pm$20.6	&24.7$\pm$20.6	&24.2$\pm$20.6	&23.6$\pm$20.4	&21.1$\pm$19.8\\
Gina	&3153	&970	&87.54	&330.8	&24.0	&164.5	&14.4$\pm$6.4	&14.3$\pm$6.5	&14.3$\pm$6.5	&14.2$\pm$6.5	&14.1$\pm$6.6	&12.5$\pm$6.5\\
Gina-p	&3168	&970	&86.77	&375.4	&21.1	&186.7	&13.4$\pm$4.7	&13.3$\pm$4.7	&13.2$\pm$4.7	&13.2$\pm$4.7	&13.1$\pm$4.8	&11.5$\pm$4.6\\
Gina-a	&3468	&784	&85.29	&373.4	&24.6	&186.0	&13.9$\pm$5.9	&13.8$\pm$6.0	&13.8$\pm$6.0	&13.7$\pm$6.1	&13.7$\pm$6.1	&12.2$\pm$6\\
Gisette	&7000	&5000	&93.67	&347.6	&36.0	&173.3	&25.2$\pm$10.4	&25.0$\pm$10.5	&25.0$\pm$10.5	&25.0$\pm$10.5	&24.8$\pm$10.6	&2.6$\pm$10.7\\
Madelon	&2600	&500	&76.00	&365.8	&17.6	&181.9	&10.6$\pm$3.5	&10.4$\pm$3.6	&10.4$\pm$3.6	&10.4$\pm$3.6	&10.3$\pm$3.6	&8.9$\pm$3.7\\
Malware	&6248	&1084	&99.09	&88.0	&11.1	&43.0	&7.3$\pm$1.6	&7.1$\pm$1.4	&7.1$\pm$1.4	&6.7$\pm$1.4	&6.4$\pm$1.3	&4.9$\pm$1.2\\
p53mutant	&31420	&5407	&99.36	&171.2	&38.9	&85.1	&37.4$\pm$4.7	&37.4$\pm$4.8	&37.4$\pm$4.8	&37.4$\pm$4.8	&37.4$\pm$4.8	&35.4$\pm$4.8\\
Pd-speech	&756	&755	&81.10	&89.6	&16.2	&44.3	&11.2$\pm$5.2	&10.9$\pm$5.3	&10.9$\pm$5.3	&10.8$\pm$5.3	&10.6$\pm$5.2	&9.4$\pm$5.3\\
Reuters	&2000	&249	&92.05	&193.0	&25.4	&89.8	&16.7$\pm$6.3	&16.4$\pm$6.3	&16.4$\pm$6.2	&16.4$\pm$6.3	&16.2$\pm$6.4	&14.2$\pm$5.9\\
Shuttle	&58000	&9	&99.98	&65.6	&9.0	&32.3&7.2$\pm$1.7	&7.2$\pm$1.7	&7.2$\pm$1.7	&7.2$\pm$1.7	&7.2$\pm$1.7	&6.2$\pm$1.6\\
Spambase	&4601	&58	&92.05	&530.4	&32.3	&261.1	&15.9$\pm$6.3	&15.3$\pm$6.1	&15.4$\pm$6.1	&14.9$\pm$6.1	&14.5$\pm$6	&11.9$\pm$5.4\\
\bottomrule
\end{tabular}
\end{center}
\end{scriptsize}
 \caption{\label{tab:results}Results for $20$ datasets. For each dataset, we indicate the number of instances (\#I), the number of features (\#F),
 the mean accuracy over the $10$ decision trees (\%A) that have been generated, the average number of nodes in those trees (\#N), their maximal depth in average (\#MD)
 the average number of binary features they are based on (\#B). The average and standard deviation is provided for  direct reasons (\#DR),  sufficient reasons (\#SR),
  minimal reasons (\#MR) and  95\% / 90\% / 75\%-probable reasons (\#95-PR / \#90-PR / \#75-PR).}
\end{table*}

 
%The empirical protocol was as follows. 
We have considered 90 datasets, which are standard benchmarks from the well-known repositories Kaggle\footnote{\url{www.kaggle.com}}, OpenML\footnote{\url{www.openml.org}}, 
and UCI\footnote{\url{archive.ics.uci.edu/ml/}}. Due to space constraints, the complete list of benchmarks used is reported as a supplementary material, 
together with additional information about the decision trees and the sizes of the different reasons that have been computed.
Several datasets considered in our experiments include a large number of instances with a large number of features.     
Because some datasets are suited to the multi-label classification task, we used the standard ``one versus all'' policy to deal with them: 
all the classes but the target one are considered as the complementary class of the target.
Categorical features have been treated as arbitrary numbers (the scale is nominal). 
As to numeric features, no data preprocessing has taken place: these features have been binarized on-the-fly 
by the decision tree learning algorithm that has been used.

% further details about the corresponding trees and 
%the computations of the various notions of reasons considered in the paper.
% Some of the datasets gather large numbers of instances, based on large numbers of features (see Table \ref{tab:results} for details).
%For example, the dataset "Dexter" contains $2600$ instances, based on $20 000$ features, and the dataset "p53 mutant" contains $16772$ instances based on $5409$ attributes.
% Some of them concern more than one class (and its complementary class).  To deal with such datasets, a ``one versus al'' policy 
% has been considered:  all the classes but the target one are considered as the complementary class of the target.
% Categorical features are treated as arbitrary numbers (the scale is nominal). As to numeric features, no preprocessing has taken place,
% all numeric features have been binarized on-the-fly by the algorithm used for generating decision trees.

For every benchmark $b$, a $10$-fold cross validation process has been achieved. 
Namely, a set of $10$ decision trees $T_b$ have been computed and evaluated
from the labelled instances of $b$, partitioned into $10$ parts. 
One part was used as the test set and the remaining $9$ parts as the training set for generating
a decision tree. This tree is thus in 1-to-1 correspondence with the test set chosen within the whole dataset $b$.
The classification performance for $b$ was measured as the mean accuracy obtained over the $10$ decision trees
generated from $b$. For the decision tree learner, we have used the CART algorithm, 
and more specifically its implementation provided by the \textrm{Scikit-Learn}\footnote{scikit-learn.org/stable/index.html} 
library. %\cite{scikit-learn} --> Ce serait bien de les citer, mais par équité ce serait bien aussi de citer les auteurs de Pysat :-)
%\footnote{\url{scikit-learn.org/stable/modules/generated/sklearn.tree.DecisionTreeClassifier.html}} 
All hyper-parameters of the learning algorithm have been set to their default value.
Notably, decision trees have been learned using the Gini criterion, and without any maximal depth or any other manual limitation. 

% using a Python  3.7.9 program based on the Scikit-Learn library, release 0.23.2\footnote{\url{https://scikit-learn.org/stable/}}. 
% The "DecisionTreeClassifier" class of this library (\url{https://scikit-learn.org/stable/modules/generated/sklearn.tree.DecisionTreeClassifier.html}) 
% has been used, each parameter being set to its default value. Especially, the Gini criterion was considered to build the decision trees.
% No maximal depth or any other manual limitation was preset. 

For each benchmark $b$, each decision tree $T_b$, and each instance $\vec x$ of the corresponding test set, 
we computed the direct reason for $\vec x$ given $T_b$, a sufficient reason for $\vec x$ given $T_b$, 
a minimal reason for $\vec x$ given $T_b$, and $\delta$-probable reasons for $\vec x$ given $T_b$ for several values of 
$\delta$ ($95\%$, $90\%$, $75\%$). 
The sufficient reason and the $\delta$-probable reasons were computed from the direct reason. % for $\vec x$ given $T_b$. % and/or from a minimal reason for $\vec x$ given $T_b$.
For computing minimal reasons, we used the Pysat\footnote{\url{https://pysathq.github.io/}} library, which provides the implementation of the RC2 \textsc{Partial MaxSAT} solver.
This solver was run using the parameters corresponding to the ``Glucose'' setting.
For each instance in a dataset and each type of reason, we computed the mean size of the reason 
(given as a number of binary features), together with the corresponding standard deviation.
In our experiments, we have also measured the runtimes required to compute any reason.
All the experiments have been conducted on a computer equipped with 
Intel(R) Core(TM) i9-9900 CPU @ 3.10 GHz  and 64 GiB of memory. 
%The kernel used was CentOS 7, Linux version 3.10.0-514.16.1.el7.x86\_64. 
%The compiler used was gcc version 5.3.1.
%Hyperthreading was disabled, and no cache share between cores was allowed.
%A time-out (TO) of 1h and a memory-out (MO) of 7.6 GiB has been considered for each instance. 

%For each benchmark $b$, all the elements of the dataset have been considered as instances $\vec x$.
%For every $\vec x$, the corresponding direct reason $p_{\vec x}^{T_b}$ given $T_b$ has been computed. We have also
%computed a sufficient reason for $\vec x$ given $T_b$ (starting the greedy algorithm on $p_{\vec x}^{T_b}$), and
%a minimal reason for $\vec x$ given $T_b$. Finally, for several values of $\delta$ ($95\%$, $90\%$, and $75\%$)\pierre{Vérifier} {\color{magenta} Steve : Tout me semble correcte, en revanche cela est un peu redondant avec la fin de mon paragraphe, il faudra sans doute fusionner les 2 explications}, we have
%computed a $\delta$-probable reason for $\vec x$ given $T_b$ (starting the greedy algorithm on the direct reason / the minimal
%reason \pierre{Vérifier} for $\vec x$ given $T_b$ that were computed previously). For every benchmark $b$, we have made some statistics about the sizes of 
%the reasons that have been computed when $\vec x$ varies in the dataset, and the computation times required to derive such reasons.

%For each benchmark, we took advantage of the Scikit-Learn to generate a decision tree \pierre{give more details, how many instances have been used, add references}.
%Then we picked up at random following a uniform distribution a set of instances $\vec x$ from the dataset such that this set contains 10\%
%of the total number of instances of the search space. For each instance $\vec x$, we have computed a corresponding reason for each notion of reason 
%(here, direct reasons, sufficient reasons, minimal reasons, and $\delta$-probable reasons) and we have measured its size. Figure \ref{???} 
%synthesizes using box plots the distribution of the sizes of the reasons for several benchmarks.
%
%If significant, one can also use scatter plots for some benchmarks (each dot corresponds to an $\vec x$, the size of its direct reason (for instance) is 
%represented on the $x$-axis and the size of its minimal reason (for instance) is represented on the $y$-axis).
%Is there a difference when focusing on instances that are misclassified by the decision tree?
%
%Discuss the obtained results.
%
%Figure \ref{???} presents using box plots the distribution of the computation times needed to extract a minimal reason from a direct reason
%for several benchmarks. For all the other notions of reasons, the computation times appear as negligible \pierre{Give more details.} 
%Discuss the results and the feasibility of the approach from the practical side.

%
%
%\begin{figure*}
% \includegraphics[width=0.5\textwidth]{farm-ads.png}
% \hfill
% \includegraphics[width=0.5\textwidth]{ad-data.png}
%  \begin{minipage}{0.5\textwidth}\centering Farm-ads\end{minipage}
%  \hfill\begin{minipage}{0.5\textwidth}\centering Ad-data\end{minipage}
% \caption{\label{fig:scatter}Comparison, for Farm-ads and Ad-data, between direct and sufficient reason (resp. 75\%-probable reason). Each dot represents
% an instance, the $x$-axis gives the size of its direct reason and the $y$-axis gives the size of the sufficient reason (resp. 75\%-probable reason) computed from the
% direct reason.}
% \end{figure*}

\subsection{Results}

Table \ref{tab:results} reports an excerpt of our results, focusing on $20$ benchmarks out of $90$ (the selected datasets
are among those containing many instances and/or many features). The leftmost column gives the name of the dataset $b$, and 
the next two columns make precise its number of instances and its number of features. 
The four following columns are about the decision trees $T_b$ that have been learned,
by indicating their mean accuracy, %(i.e., the mean accuracy over the $10$ decision trees associated with $b$), --> on l'a déjà écrit plus haut !
the average number of their nodes, their maximal depth in average, and the average number of binary features they are built on.
The next columns give the results obtained for the direct reason, the sufficient reason, the minimal reason, the $95\%$-probable
reason, the $90\%$-probable reason, and finally the $75\%$-probable reason. 
For each reason, we have reported its average size, together with its standard deviation.% and its maximal size encountered on test instances.

% for the different reasons, their average size, 
%  at hand, their average size of the reasons. 
% The corresponding standard deviation is also provided, as well as the maximal size encountered.
% Those measurements are successively presented for the direct reason, the sufficient reason, the minimal reason, the $95\%$-probable
% reason, the $90\%$-probable reason, and finally the $75\%$-probable reason.% (\gilles{on peut enlever ces explications, si on les laisse dans la légende du tableau.}])

\begin{figure*}
\begin{center}
\scalebox{0.8}{
\includegraphics[width=0.5\textwidth]{farm-ads.png}
\hfill
\includegraphics[width=0.5\textwidth]{ad-data.png}
}
 \caption{\label{fig:scatter} Comparison, for Farm-ads (left) and Ad-data (right), between the sizes of direct reasons vs. the sizes of minimal reasons (green triangles) and
 $75\%$-probable reasons (red stars). }
 %Each dot represents
% an instance, the $x$-axis gives the size of its direct reason and the $y$-axis gives the size of the sufficient reason (resp. 75\%-probable reason) computed from the
% direct reason.}
\end{center}
\end{figure*}

In light of these results, we can observe that the direct reasons of input instances are typically far much shorter than the instances themselves.
This is a strong argument about why decision trees are typically considered as interpretable models. 
Yet, when switching to the other types of reasons examined in the paper, some additional features are often removed. 
%By construction, the resulting explanations cannot be larger than the direct reasons, and as such, 
%they are at least as intelligible as the reasons computed directly from decision trees. 
It is interesting to note that the reductions that are achieved (in number of literals) 
are more salient for the $\delta$-probable reasons (in particular, when $\delta = 75\%$) than for the minimal reasons. 
Empirically, it turns out that for many instances $\vec x$, the direct reason for $\vec x$ is actually a minimal reason, 
or an ``almost minimal'' one, in the sense that it contains very few irrelevant features for classifying $\vec x$.
Though the suppression of irrelevant (or ``probably irrelevant'') features in reasons is not enough to guarantee that 
the size of the reasons will always stay below the cognitive barrier of $7 \pm 2$ features (as pointed out by George Miller), especially 
when dealing with high-dimensional classification tasks,  this objective has been reached by the direct reasons for
$68$ out of $90$ benchmarks used in the experiments.

In order to figure out the benefits obtained when switching from direct reasons 
to other reasons, we drew a number of scatter plots: each instance $\vec x$ of $b$ corresponds to a point,
its $x$-coordinate gives the size of its direct reason, and its $y$-coordinate 
gives the size of the minimal reason (or of the $75\%$-probable reason) that has been computed.  
Figure~\ref{fig:scatter} gives such scatter plots for the benchmarks ``Add-data'' and ``Farm-ads''.
Here, we can observe that a significant reduction of the number of features used in the direct reasons may occur. 
Specifically, for minimal reasons, the average reduction of the size of the direct reasons achieved for ``Add-data'' 
(resp. ``Farm-ads'' )  was of  $11.5\%$ (resp. $3.5 \%$) while the maximal reduction for ``Add-data''  (resp. ``Farm-ads'') 
was of  $65.2\%$ (resp. $76.2\%$). For $75\%$-probable reasons, the average reduction of the size 
of the direct reasons achieved for ``Add-data'' (resp. ``Farm-ads'') was of  $32.9\%$ (resp. $22\%$) while the
maximal reduction for ``Add-data'' (resp. ``Farm-ads'') was of  $100\%$  (resp. $90\%$). 
Interestingly, for ``Add-data'', the sizes of minimal reasons (resp. $75\%$-probable reasons) 
never exceeded $37$ (resp. $106$) regardless of the size of direct reasons.

% In order to figure out the benefits in term of reduction of the number of features 
% that are obtained when switching from direct reasons to the other notions of reasons,
% we drew a number of scatter plots, where for each instance $\vec x$ of $b$, the size of the corresponding direct reason is reported on the $x$-axis
% and the size of the $75\%$-probable reason that has been computed for $\vec x$
% is reported on the $y$-axis. Figure~\ref{fig:scatter} gives such scatter plots for the benchmarks ``Add-data'' and ``Farm-ads''.
% We can observe on this figure that a significant reduction of the number of features used in the direct reasons may occur. Thus, 
% as to minimal reasons, the average reduction of the size of the direct reasons achieved for ``Add-data'' (resp. ``Farm-ads'') was of  $?? \%$ (resp. $?? \%$) while the
% maximal reduction for ``Add-data'' (resp. ``Farm-ads'') was of  $?? \%$ (resp. $?? \%$). As to $75\%$-probable reasons, the average reduction of the size 
% of the direct reasons achieved for ``Add-data'' (resp. ``Farm-ads'') was of  $?? \%$ (resp. $?? \%$) while the
% maximal reduction for ``Add-data'' (resp. ``Farm-ads'') was of  $?? \%$  (resp. $?? \%$). For ``Add-data'',  the sizes of the minimal reasons
% (resp. $75\%$-probable reasons) never exceeded $??$ (resp $??$) whatever the size of the direct reasons.

\begin{figure}[h]
\scalebox{0.8}{
\includegraphics[width=0.5\textwidth]{decrease-proba.png}
}
 \caption{\label{fig:decrease}Average size of $\delta$-probable reasons when $\delta$ varies from $1$ (sufficient reasons) to $0.5$ for the datasets ``Madelon'', ``Malware'', and ``Spambase''.}
\end{figure}

Finally, since the reduction of the size of the reasons achieved by considering $75\%$-probable reasons in comparison to direct reasons
looked significant, we have also run additional experiments in order to get a clearer picture of the reduction that can be achieved
when $\delta$ varies. We have computed the sizes of the $\delta$-probable reasons of instances while $\delta$ varies from
$100\%$ (in this case, $\delta$-probable reasons correspond to sufficient reasons) to $50\%$.  Figure \ref{fig:decrease} reports such plots for the benchmarks
``Madelon'', ``Malware'', and ``Spambase''.  As expected, one can observe that the mean size of the $\delta$-probable reasons smoothly decreases %in quite a smooth way 
when $\delta$ diminishes.

As to the computation times, it turns out that all the algorithms used for deriving reasons proved very efficient in practice 
(despite the use of a fully-interpreted version of Python for the implementation). Indeed, for every benchmark $b$ but ``Adult'', and every instance $\vec x$ of $b$, 
a reason for $\vec x$ given $T_b$ has been generated {\bf in less than 100ms}, whatever the type of reason one was looking for. 
Note that ``Adult'' led to quite huge decision trees
(in average, with $12926$ nodes, based on more than $2973$ binary features). Despite this size, for this dataset, the computation times for
computing a reason never exceeded $600$ms, except for minimal reasons which turned out to be more demanding from a computation point of view (as
this was expected in light of Proposition \ref{prop:minimalreasonDT}). But it is worth noting that even the performance of the algorithm for 
computing minimal reasons was not that bad for this benchmark, with an average computation time of $2.69$s and a maximal computation time of $5.06$s.
This explains why we have refrained from leveraging Proposition \ref{prop:approximable} to compute approximate minimal reasons.
%At a first glance, the empirical efficiency of the algorithm for computing minimal reasons was a surprise, 
%given the intrinsic complexity of the derivation of minimal reasons. However, the progress made in \textsc{SAT} solving 
%for the past two decades explains why our empirical results are finally not that surprising. 
%%, such an a priori judgement must be taken with a pinch of salt, as our empirical results confirm it.

%\color{black}

==> introduction.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In essence, explaining a decision to a person is to give the details or \emph{reasons} that help the person 
understand why the decision has been made. This is a significant issue 
especially when decisions are made by Machine Learning (ML) models, such as random forests, Markov networks,
support vector machines, and deep neural networks. Actually, with the growing number of applications that rely on ML techniques, 
researches on eXplainable AI (XAI) have become increasingly important, by providing efficient methods for 
interpreting ML models, and explaining their decisions 
(see for instance \cite{DBLP:conf/aiia/FrosstH17,GuidottiMRTGP19,Hooker19,Huysmans11,DBLP:conf/aaai/IgnatievNM19,Kim18,Lundberg17,DBLP:journals/ai/Miller19,Molnar19,Ribeiro16,DBLP:conf/sat/ShihDC19}).  


% This is a significant issue, especially when decisions are generated automatically by AI systems, 
% inclluding classifiers and other machine learning (ML) models.  
% In the context of classification, the decision to be explained is the concept (class) that is predicted
% from the input instance.

% Of course, deriving explanations calls for dedicated technologies. Given the importance
% of the issue, there has been a growing body of work on explainable and robust AI (XAI) for the past couple of years 
% (see for instance \cite{DBLP:conf/aaai/IgnatievNM19,DBLP:conf/nips/BunelTTKM18,DBLP:journals/corr/abs-1805-09938,DBLP:journals/jossw/MolnarCB18,DBLP:conf/sat/ShihDC19,GuidottiMRTGP19,DBLP:journals/ai/Miller19,Molnar19}). 
% \pierre{This list must be updated.}

For classification problems, \emph{decision trees} \cite{DBLP:books/wa/BreimanFOS84,DBLP:journals/ml/Quinlan86} are models of 
paramount importance in XAI, as they can be easily read by recursively breaking a choice into sub-choice until a decision is reached.
Although there is no formal notion of \emph{interpretability} \cite{DBLP:journals/cacm/Lipton18}, decision trees are arguably among 
the most interpretable ML models, endowed with two key characteristics. On the one hand, decision trees are \emph{transparent}: 
each node in a decision tree has some meaning, and the principles used for generating all nodes can be explained.  
On the other hand, decision trees are \emph{locally explainable}: by construction of a decision tree, 
any input instance $\vec x$ is mapped to a unique root-to-leaf path $p$ that yields to a decision $y$. 
The subset of features occurring in $p$ can be viewed as a ``direct reason'' for classifying $\vec x$ as $y$. 
Because of their interpretability, decision trees are often considered are target models for distilling a black-box model into 
a comprehensible one \cite{BreimanShang96,DBLP:conf/aiia/FrosstH17}. Furthermore, decision trees are often the components of choice  
for building (less interpretable, but potentially more accurate) ensemble classifiers, 
such as random forests \cite{DBLP:journals/ml/Breiman01} and gradient boosted decision trees \cite{Chen16}.  


% labeled by some decision tree, one can easily get a ``direct reason''  for ,  
% i.e., a subset $p$ of the characteristics of $\vec x$ such that every instance $\vec x'$ sharing this subset 
% $p$ would be classified in the same way as $\vec x$. The set $p$ corresponds to the (unique) path of the decision tree that is 
% compatible with $\vec x$. The set $p$ can be computed efficiently (that is, in time linear in the size of the input). Furthermore, $p$ can be considered as a better explanation of the prediction made for $\vec x$ than $\vec x$ itself because $p$ contains (often) less characteristics than $\vec x$.


% While there is no formal definition of what an interpretable ML model should be \cite{DBLP:journals/cacm/Lipton18}, decision trees are usually considered 
% as interpretable. There are two main justifications for it. 
% On the one hand, the \emph{decomposability property} of decision trees: each node in a decision tree has some meaning, and the principles used for generating
% a decision tree can be justified. On the other hand, the \emph{local explanation facility} they provide:  from any instance $\vec x$ to be classified and a decision tree used as a classifier, one can easily get, together with the class that is predicted for the instance, a ``direct reason''  for the classification of $\vec x$, i.e., a subset $p$ of the characteristics of $\vec x$ such that every instance $\vec x'$ sharing this subset $p$ would be classified in the same way as $\vec x$. The set $p$ corresponds to the (unique) path of the decision tree that is compatible with $\vec x$. The set $p$ can be computed efficiently (that is, in time linear in the size of the input). Furthermore, $p$ can be considered as a better explanation of the prediction made for $\vec x$ than $\vec x$ itself because $p$ contains (often) less characteristics than $\vec x$.

Although there is no consensus on what constitutes a ``good'' explanation 
\cite{DBLP:journals/corr/abs-1802-00682,DBLP:journals/ai/Miller19,DBLP:conf/ijcai/0002C20}, 
when it comes to explaining classification tasks, 
the notion of \emph{sufficient reasons} \cite{DarwicheHirth20} 
(also known as prime implicant explanations \cite{ShihCD18}) appears as a valuable candidate. 
A sufficient reason for an instance $\vec x$ classified as $y$ by a Boolean function $f$ is a subset $t$ of the 
features of $\vec x$ that is minimal with respect to set inclusion, and such that any instance $\vec x'$ sharing 
this set $t$ of features is also classified as $y$ by $f$.
The significance of sufficient reasons comes from Occam's razor which roughly states that the best explanations 
are the simpler ones. 
Indeed, since any sufficient reason $t$ for  is minimal w.r.t. set inclusion, it does not contain any locally irrelevant feature
for classifying $\vec x$. In other words, if $t$ is a sufficient reason for an instance $\vec x$, labeled as $y$ by the classifier $f$, then
removing any feature from $t$ would call into question the fact that $\vec x$ is classified as $y$ by $f$. 

When the Boolean function $f$ is represented by a decision tree, say $T$, the direct reason $p$ obtained 
by reading the root-to-leaf path that classifies the input instance $\vec x$ contains typically far less features than $\vec x$ itself.
However, from the theory side, it has been shown recently that $p$ may contain arbitrarily many more features 
than a sufficient reason for $\vec x$ given $T$ \cite{DBLP:journals/corr/abs-2010-11034}. 
Furthermore, from a more practical side, experiments reported in the same paper have pointed out that the number of extra features 
contained in direct reasons can be significantly larger than the size of sufficient reasons. 
Fortunately, one can take advantage of a greedy strategy to eliminate efficiently from $p$ any irrelevant feature, 
and this results in a polynomial-time algorithm for computing a sufficient reason for $\vec x$ given $T$.

Does this mean that the game is over and the question of explaining predictions from decision trees fully addressed? 
Not really: it cannot be guaranteed that the sufficient reasons computed by the greedy strategy are intelligible enough, 
because they may contain (too) many features. To this very point, it must be kept in mind that explaining is a social process \cite{DBLP:journals/ai/Miller19},
where explainees are \emph{human beings}, who (inherently) have \emph{cognitive limitations}. 
In his seminal paper \cite{Miller56}, %(that marked the beginning of cognitive psychology as a field) --> Pas certain que ce soit nécessaire ... 
Psychologist George Miller introduced the idea of people ``chunking'' items (i.e., grouping them together as a unit) and argued that
due to human memory limitations, the size of chunks is limited to 7, plus or minus 2. 
Ever since then, many experiments in cognitive science have confirmed this limitation. 
Restricting explanations to contain only few features thus appears as an important requirement 
for ensuring that they are intelligible.
So, what can be done if the sufficient reason that has been computed includes too many attributes 
for being considered as intelligible? As a step towards more intelligibility, is it possible to define well-founded 
notions of reasons requiring less attributes
than sufficient reasons?
%by the explainee

These are the main research questions considered in the paper. 
In order to go even further in the direction of characterizing and computing simple explanations,
we first consider a refinement of the notion of sufficient reasons, namely \emph{minimal reasons}, 
that focuses on explanations of minimal size.
We also consider a generalization of sufficient reasons, namely \emph{probable reasons},
for which a small proportion of models can disagree with the classification made on the input instance.
In both cases, we identify the complexity of computing a reason for a given instance 
when the classifier is a decision tree, and we describe exact or approximate algorithms 
for deriving such reasons. 
%We focus here on Boolean features \pierre{To be commented, is it without any loss of generality because other features can be binarized if needed? References are expected here.}
Finally, we report empirical results illustrating, from a practical viewpoint, the 
gain in intelligibility that is obtained via minimal reasons and probable reasons, 
and the performances of the algorithms for computing them. 

The paper is organized as follows. % \textcolor{blue}{TBC. }
Preliminaries about decision trees and sufficient reasons are given in Section \ref{formal}.
Minimal and probable reasons are defined and analyzed in Section \ref{beyond}.
Experimental results are reported in Section \ref{experiments}.
Finally, Section \ref{conclusion} concludes the paper. % and presents some perspectives for further research. 
Proofs and detailed empirical results are provided as a supplementary material. 

%
%These are the main research questions considered in the paper. Our objective is to contribute to address them.
%To this purpose, we present some refinements / generalizations of the notion of sufficient reasons.  Thus, the
%notions of \emph{comprehensible reasons} and \emph{inclusion-preferred reasons} are introduced as a contribution to the first issue, and
%notions of \emph{minimal reasons} (and more generally of \emph{minimal-weight reasons}) as a contribution to the second issue. 
%We also present a notion of  \emph{probabilistic reasons}, that  generalizes sufficient reasons and
%prove useful for both issues. 


==> preliminaries.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Decision Trees and Sufficient Reasons}\label{formal}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% \paragraph{Boolean formulae.} 
For an integer $n$, let $[n]$ be the set $\{1,\cdots,n\}$.
By $\mathcal F_n$ we denote the class of all Boolean functions from $\{0,1\}^n$ to $\{0,1\}$,
and  we use $X_n  = \{x_1, \cdots, x_n\}$ to denote the set of input Boolean variables. 
Any assignment $\vec x \in \{0,1\}^n$ is called an \emph{instance}. If $f(\vec x) = 1$ 
for some $f \in \mathcal F_n$, then $\vec x$ is called a \emph{model} of $f$.
We refer to $f$ as a propositional formula when it is described using the Boolean connectives $\land$ (conjunction), $\lor$ (disjunction) and 
$\neg$ (negation), together with the Boolean constants $1$ (true) and $0$ (false). 
As usual, a \emph{literal} $l_i$ is a variable $x_i$ or its negation $\neg x_i$, also denoted $\overline x_i$.
A \emph{term} (or \emph{monomial}) $t$ is a conjunction of literals, and a \emph{clause} $c$ is a disjunction of literals. 
A \emph{\dnf\ formula} is a disjunction of terms and a \emph{\cnf\ formula} 
is a conjunction of clauses. 
%The set of variables occurring in a formula $F$ is denoted $\Var{F}$.--> Je crois qu'on ne l'utilise plus.

In what follows, we shall often treat assignments as terms, and (consistent) terms as sets of literals. 
Given an assignment $\vec z \in \{0,1\}^n$, the corresponding term is defined as
\begin{align*}
t_{\vec z} = \bigwedge_{i=1}^n x_i^{z_i} \mbox{ where } x_i^0 = \overline x_i \mbox{ and } x_i^1 = x_i
\end{align*}
A term $t$ \emph{covers} an assignment $\vec z$ if $t \subseteq t_{\vec z}$. 
An \emph{implicant} of a Boolean function $f$ is a term that implies $f$, that is, a term $t$ such that $f(\vec z) = 1$ 
for every assignment $\vec z$ covered by $t$. 
A \emph{prime implicant} of $f$ is an implicant $t$ of $f$ such that no proper subset of $t$ is an implicant of $f$. 

% Je crois bien qu'on n'a plus besoin de cela :
%Given a propositional formula $F$ and a literal $l_i$, the \emph{conditioning} of $F$ by $l_i$,
%denoted $F \mid l_i$ is the formula obtained from $F$ by replacing each occurrence of $x_i$ with $1$ (resp. $0$) and each occurrence of $\overline x_i$
%with $0$ (resp. $1$) if $l_i = x_i$ (resp. $l_i = \overline x_i$). 


With these basic notions in hand, we shall focus on the following representation class of Boolean functions:

\begin{definition}[Decision Tree] A (Boolean) \emph{decision tree} is a binary tree $T$, each of whose internal nodes is labeled with one of
    $n$ input Boolean variables, and whose leaves are labeled $0$ or $1$. Every variable is assumed (without loss of generality) to appear at most once on any root-to-leaf path (read-once property).  
    The value $T(\vec x) \in \{0,1\}$ of $T$ on an input instance $\vec x$ is given by the label of the
    leaf reached from the root as follows: at each node, go to the left or right child depending on whether the input value of the corresponding variable is $0$ or $1$, 
    respectively. The size of $T$, denoted $\size{T}$, is given by the number of its nodes.
\end{definition}

The class of decision trees over $X_n$ is denoted $\dt_n$. 
%Obviously enough, any Boolean function in $\mathcal F_n$ can be represented by a decision tree in $\dt_n$. --> Dangereux 
% car les DT peuvent avoir une taille exponentielle.
%Note that any Boolean function in $\mathcal F_n$ can be represented by a decision tree
%in $\dt_n$ with $2^n$ leaves and depth of $n + 1$. Since the sample complexity of $\dt_n$ is exponential in $n$, most 
%theoretical results about decision trees focus on restricted subclasses, such as the class  
%$\dt^k_n$ of decision trees over $X_n$ of depth $k$.
It is well-known that any decision tree $T \in \dt_n$ can be transformed in linear time into an equivalent disjunction of terms, denoted $\dnf(T)$,
where each term corresponds to a path from the root to a leaf labeled with $1$. Dually, $T$ can be transformed in linear time into 
a conjunction of clauses, denoted $\cnf(T)$, where each clause is the negation of the term describing a path from the root to a leaf labeled with $0$.

For illustration, the following toy example will be used throughout the paper as a running example:

\begin{figure}[t]
\centering
\scalebox{0.65}{
      \begin{tikzpicture}[scale=0.6] 
        \node[ellipse,draw](root) at (7,9){$x_1$};
        \node[ellipse,draw](n1) at (2,7){$x_2$};
        \node[ellipse,draw](n2) at (12,7){$x_2$};
        \node(n11) at (1,5){$0$};          
        \node[ellipse,draw](n12) at (3,5){$x_3$};  
        \node(n121) at (2,3){$0$};  
        \node[ellipse,draw](n122) at (4,3){$x_4$};   
        \node(n1221) at (3,1){$0$}; 
        \node(n1222) at (5,1){$1$}; 
        
        \node[ellipse,draw](n21) at (9,5){$x_3$};
        \node[ellipse,draw](n22) at (15,5){$x_3$};   
        \node[ellipse,draw](n211) at (7,3){$x_4$};
        \node[ellipse,draw](n212) at (10,3){$x_4$};              
        \node[ellipse,draw](n221) at (13,3){$x_4$};
        \node[ellipse,draw](n222) at (16,3){$x_4$};   
        
        \node(n2111) at (6,1){$0$}; 
        \node(n2112) at (8,1){$1$};         
        \node(n2121) at (9,1){$0$}; 
        \node(n2122) at (11,1){$1$}; 
        \node(n2211) at (12,1){$0$}; 
        \node(n2212) at (14,1){$1$}; 
        \node(n2221) at (15,1){$0$}; 
        \node(n2222) at (17,1){$1$}; 
                               
        \draw[densely dotted] (root) -- (n1);
        \draw(root) -- (n2);
        \draw[densely dotted] (n1) -- (n11);
        \draw(n1) -- (n12);       
        \draw[densely dotted] (n12) -- (n121);
        \draw(n12) -- (n122); 
        \draw[densely dotted] (n122) -- (n1221);
        \draw(n122) -- (n1222); 
        
        \draw[densely dotted] (n2) -- (n21);
        \draw(n2) -- (n22);    
        \draw[densely dotted] (n21) -- (n211);
        \draw(n21) -- (n212);                
        \draw[densely dotted] (n22) -- (n221);
        \draw(n22) -- (n222);  
        \draw[densely dotted] (n211) -- (n2111);
        \draw(n211) -- (n2112);
        \draw[densely dotted] (n212) -- (n2121);
        \draw(n212) -- (n2122);    
        \draw[densely dotted] (n221) -- (n2211);
        \draw(n221) -- (n2212);
        \draw[densely dotted] (n222) -- (n2221);
        \draw(n222) -- (n2222);  
      \end{tikzpicture}
 }
    \caption{A decision tree $T$ for recognizing {\it Cattleya} orchids. The left (resp. right) child of any decision node labelled by $x_i$ corresponds to 
    the assignment of $x_i$ to $0$ (resp. $1$).\label{fig:orchids}}
    \end{figure}

\begin{example}\label{running-ex}
The decision tree in Figure \ref{fig:orchids} separates {\it Cattleya} orchids from other orchids using the following features:
\begin{itemize}
\item $x_1$: ``has fragrant flowers'';
\item $x_2$: ``has one or two leaves'';
\item $x_3$: ``has large flowers'';
\item $x_4$: ``is sympodial'';
\item $x_5$: ``has white flowers''.
\end{itemize}
By construction, $\overline x_1 \land  x_2 \land x_3 \land x_4$ is a term of $\dnf(T)$, and 
$x_1 \lor x_2$ is a clause of $\cnf(T)$. Note that $x_5$ is a (globally) irrelevant feature since it does not appear 
in any path of $T$.
\end{example}

The key focus of this study is to explain \emph{why} a decision tree $T \in \dt_n$
classifies an incoming instance $\vec x$ as positive. 
A \emph{reason} for $T(\vec x) = 1$ typically takes the form of conjunction of literals 
which together justify the prediction made by $T$ on $\vec x$. 
We mention in passing that focusing on the case $T(\vec x) = 1$ is without any loss of generality  
because $\dt_n$ is closed under negation.\footnote{For any $T \in \dt_n$, $\neg T$ is obtained 
by just replacing from $T$ the label of each leaf with its complement. 
So, a reason why $T(\vec x) = 0$ is precisely the same as a reason why $(\neg T)(\vec x) = 1$.}
As a salient characteristic, decision trees convey a single explicit explanation for classifying any input instance:  
%for decision trees since (i) a reason why  $T(\vec x) = 0$ is precisely the same as a reason why $(\neg T)(\vec x) = 1$, 
%and (ii) $\neg T$ is the decision tree obtained from $T$ by just replacing the label of each leaf.
%(see e.g. \cite{Koricheetal13}) --> Pas besoin de citer c'est trivial et il est déjà connu que DT est clos par complémentation.


%As stressed in the introduction, decision trees are models of paramount importance in XAI, as they can be easily read by 
%recursively breaking a choice into sub-choice until a decision is reached. Notably, decision trees convey 
%a single explicit explanation for classifying any input instance:      
%--> C'est la caractéristique principale des DT, je pense qu'il faut mettre ce paragraphe directement en intro.

\begin{definition}[Direct Reason] 
    Let $T \in \dt_n$ and $\vec x \in \{0,1\}^n$ such that $T(\vec x) = 1$.
    The \emph{direct reason} for $\vec x$ given $T$ is the term, denoted $p_{\vec x}^T$, 
    corresponding to the unique root-to-leaf path of $T$ that is compatible with $\vec x$. 
\end{definition}

%In the context of Boolean classification, every variable $x_i \in X_n$ is referred to as a \emph{feature}, 
%and a literal based on $x_i$ (reflecting the fact that $x_i$ is assigned to $0$ or $1$) is called a \emph{characteristic}.
%Every assignment $\vec x \in \{0,1\}^n$ is an \emph{instance}. $\vec x$ is classified as an element of the concept represented
%by $T$ if and only if $T(\vec x) = 1$. ---> Fred : on n'a pas besoin de ces notions élémentaires en ML. D'autre part, éviter le 
% terme "characteristic" qui est utilisé pour tout autre chose en ML.

\begin{example}
Based on our running example, we can observe that $T(\vec x) = 1$ for the instance $\vec x = (1, 1, 1, 1, 1)$.
The direct reason for $\vec x$ given $T$ is the term $p_{\vec x}^T = x_1 \land x_2 \land x_3 \land x_4$. 
\end{example}

% As the previous definition illustrates it, the key focus of this study is to explain \emph{why} $T$ classifies $\vec x$ as \emph{positive}. 
% The reasons for explaining $T(\vec x) = 1$ typically take the form of a conjunction of literals which together justify the prediction 
% made by $T$ on $\vec x$.  We mention in passing that focusing on $T(\vec x) = 1$ is without any loss of generality for decision trees
% since (i) a reason why  $T(\vec x) = 0$ is precisely the same as a reason why $(\neg T)(\vec x) = 1$, and (ii) 
% any decision tree $T \in  \dt_n$ can be transformed in linear time into a decision tree $T' \in \dt_n$ 
% that is equivalent to $ \neg T$. Indeed, the decision tree $T'$ obtained from $T$ by replacing the label of each leaf 
% with its complement is equivalent to $\neg T$(see e.g. \cite{Koricheetal13}).

Another important notion when dealing with the explanation of predictions is the following:

\begin{definition}[Sufficient Reason] 
    Let $f \in \mathcal F_n$ and $\vec x \in \{0,1\}^n$ such that $f(\vec x) = 1$.
    A \emph{sufficient reason} for $\vec x$ given $f$ is a prime implicant $t$ of $f$ that covers $\vec x$.
\end{definition}

% \begin{definition}[Sufficient Reason] 
%     Let $f \in \mathcal F_n$ and $\vec x \in \{0,1\}^n$ such that $f(\vec x) = 1$.
%        A \emph{sufficient reason} for $\vec x$ given $f$ is a prime implicant $t$ of $f$ which is implied by $\vec x$, that is, 
%     $t$ is a subset-minimal set of literals from $\vec x$ for which any instance containing it is a model of $f$.
% \end{definition}

\begin{example}%[Example \ref{running-ex} cont'ed]
In our running example, $x_2 \wedge x_3 \wedge x_4$ is a sufficient reason for $\vec x$ given $T$.
It is a better explanation than the direct reason $p_{\vec x}^T = x_1 \wedge x_2 \wedge x_3 \wedge x_4$, since 
$x_1$ is redundant (locally irrelevant) in the direct reason for $\vec x$. 
\end{example}

For the class $\dt_n$, it is already known that sufficient reasons 
can be found in polynomial time (see e.g., \cite{DBLP:journals/corr/abs-2010-11034}).
More precisely, given $T \in \dt_n$ and $\vec x \in  \{0,1\}^n$ such that $T(\vec x) = 1$, 
one can return in $\mathcal O(\size{T}n)$ time a sufficient reason $t$ for $\vec x$ given $T$ 
using the following greedy algorithm (that is reminiscent to the one considered in \cite{Schrag96} for a knowledge 
compilation purpose): start with $t = t_{\vec x}$, and iterate over the literals $l_i$ of 
$t$ by checking whether $t$ deprived of $l_i$ is an implicant of $T$.\footnote{This can be done in $O(\size{T})$ time 
by checking whether $t \setminus \{l_i\}$ is an implicant of $\cnf(T)$.}  
If so, remove $l_i$ from $t$ and proceed to the next literal.
Once all literals in $t_{\vec{x}}$ have been examined, the final term $t$ is by construction an implicant of $T$ such that
removing any literal from it would lead to a term that is not any longer an implicant of $T$. Thus, $t$
is a prime implicant of $T$ containing only literals from $\vec{x}$.
Clearly enough, instead of starting the greedy algorithm with $t = t_{\vec x}$, one may consider 
any implicant of $T$ that covers $\vec x$. In particular, the greedy algorithm can be run 
on $t = p_{\vec x}^T$. %, the direct reason for $\vec x$ given  $T$.

%Finally, it is worth noting that the problem of deriving \emph{all} sufficient reasons for
%a given instance is much more demanding in general. Indeed, even for the restricted class of decision trees with
%logarithmic depth, an input instance can have exponentially many sufficient reasons:
%
%\begin{proposition}\label{prop:nbDT}
%There is a decision tree $T \in\dt_n$ of depth $\log_2(n + 1)$ 
% such that for any $\vec x \in \{0,1\}^n$, the number of sufficient reasons for $\vec x$ given $T$ is at least 
% $\lfloor \frac{3}{2}^{\frac{n + 1}{2}} \rfloor$. 
%\end{proposition}

% Deciding whether any term $t$ included in $\vec x$ is an implicant of $T$ is equivalent to checking whether 
% $t$ entails $\cnf(T)$, which can be done in $O(\size{T})$ time. 
% Thus, by performing this implicant test $n$ times, the runtime of the greedy algorithm is in $\mathcal O(\size{T}n)$.

% The key task of the greedy algorithm is to decide whether any term $t$ included in $\vec x$  is an 
% implicant of $T$, which is equivalent to check whether $T \mid t$ (the conditioning of $T$ by $t$) 
% is a decision tree with no leaves labeled by $0$. To this point, $T \mid t$ can be constructed in $O(\size{T})$
% time using the following procedure: sort all internal vertices of $T$ in reverse topological order and, 
% for each vertex $v_i$ in that order, check whether the corresponding variable $x_i$ 
% occurs as a literal $l_i$ of $t$\footnote{This can be done in $\mathcal O(1)$ time using a vector encoding of $t$.}. 
% If so, replace the node $v_i$ by its right child if $l_i = x_i$, and its left child if $l_i = \overline x_i$.
% By performing this implicant test $n$ times, the runtime of the greedy algorithm is in $\mathcal O(\size{T}n)$.

% which returns as output a sufficient reason $t$ for $\vec x$ given $T$ in $\mathcal O(n \size{T})$ time.
% \footnote{Note that this algorithm can be extended easily to the case of random forests without questioning its tractability.}
% The tractability of finding sufficient reasons in decision trees lies in the fact that deciding whether a consistent term $t$ is an implicant 
% of a decision tree $T$ can be obtained by checking whether $T \mid t$ (the conditioning of $T$ by $t$) 
% is a decision tree with no leaves labeled by $0$. Notably, $T \mid t$ can be computed in $\mathcal O(\size{T} \size{t})$ 
% time by iteratively conditioning $T$ by each literal occurring in $t$. For any such literal $l_i$ with variable $x_i$,
% $T \mid l_i$ is obtained by simply replacing each internal node $x_i$ in $T$ with its right child if $l_i = x_i$, 
% and its left child if $l_i = \overline x_i$.
    % With this implicant test in hand, the generation of a sufficient reason for $\vec x$ given $T$ 
% can be found using the following greedy algorithm: start with $t = \vec x$, and iterate over the literals $l_i$ of 
% $t$ by checking whether $t$ deprived of $l_i$ is still an implicant of $T$. 
% If so, remove $l_i$ from $t$ and proceed to the next literal.
% Once all the variables $\vec{x}$ have been examined, the term $t$ is by construction an implicant of $T$ such that
% removing any literal from $t$ would lead to a term that is not any longer an implicant of $T$. Thus, $t$
% is a prime implicant of $T$ and it contains only literals from $\vec{x}$.

